Towards more transferable adversarial attack in black-box manner

Adversarial attacks have become a well-explored domain, frequently serving as evaluation baselines for model robustness. Among these, black-box attacks based on transferability have received significant attention due to their practical applicability in real-world scenarios. Traditional black-box methods have generally focused on improving the optimization framework (e.g., utilizing momentum in MI-FGSM) to enhance transferability, rather than examining the dependency on surrogate white-box model architectures. Recent state-of-the-art approach DiffPGD has demonstrated enhanced transferability by employing diffusion-based adversarial purification models for adaptive attacks. The inductive bias of diffusion-based adversarial purification aligns naturally with the adversarial attack process, where both involving noise addition, reducing dependency on surrogate white-box model selection. However, the denoising process of diffusion models incurs substantial computational costs through chain rule derivation, manifested in excessive VRAM consumption and extended runtime. This progression prompts us to question whether introducing diffusion models is necessary. We hypothesize that a model sharing similar inductive bias to diffusion-based adversarial purification, combined with an appropriate loss function, could achieve comparable or superior transferability while dramatically reducing computational overhead. In this paper, we propose a novel loss function coupled with a unique surrogate model to validate our hypothesis. Our approach leverages the score of the time-dependent classifier from classifier-guided diffusion models, effectively incorporating natural data distribution knowledge into the adversarial optimization process. Experimental results demonstrate significantly improved transferability across diverse model architectures while maintaining robustness against diffusion-based defenses.

==> table/editing_image_quality.tex <==
\begin{table}[]
    \centering
    \caption{Comparison of our proposed method with baseline methods in terms of Image Quality
Assessment (IQA) metrics. Here is comparing between purified clean image and purified adversarial image.  Arrows ($\uparrow$/$\downarrow$) indicate whether higher or lower values represent
better image quality for each image quality metric.}
    \begin{tabular}{c|ccc|ccc}
    \toprule
    & &  $\gamma=16/255$& &&$\gamma=8/255$  &  \\
    \midrule
    Method& SSIM $\uparrow$ &  PSNR $\uparrow$& LPIPS $\downarrow$& SSIM $\uparrow$ &  PSNR $\uparrow$& LPIPS $\downarrow$ \\
    \midrule
        PGD & 0.8745& 30.03&0.1472 & 0.8869&  30.28&0.1301\\
   
        Diff-PGD~\cite{xue2023diffusion} &{0.8661}&{29.81}&{0.1634} &0.8846& 30.21& 0.1340
        \\
        \midrule
        Score(Ours) & \textbf{0.8592}& \textbf{29.19} &\textbf{0.1799}& \textbf{0.8803}& \textbf{29.89}& \textbf{0.1444}
        \\
        Score+CE (Ours) & \textbf{0.8592}& \textbf{29.19} &\textbf{0.1799}& \textbf{0.8803}& \textbf{29.89}& \textbf{0.1444}
        \\
        \bottomrule
    \end{tabular}
    
    \label{tab:IQA for purify image}
\end{table}
